MPGemmFI: A Fault Injection Technique for Mixed Precision GEMM in ML Applications

Emerging deep learning workloads urgently need fast general matrix multiplication (GEMM). To meet such demand, one of the critical features of machine-learning-specific accelerators such as NVIDIA Tensor Cores, AMD Matrix Cores, and Google TPUs is the support of mixed-precision enabled GEMM. For DNN models, lower-precision FP data formats and computation offer acceptable correctness but significant performance, area, and memory footprint improvement. While promising, the mixed-precision computation on error resilience remains unexplored. To this end, we develop a fault injection framework that systematically injects fault into the mixed-precision computation results. We investigate how the faults affect the accuracy of machine learning applications. Based on the error resilience characteristics, we offer lightweight error detection and correction solutions that significantly improve the overall model accuracy if the models experience hardware faults. The solutions can be efficiently integrated into the accelerator's pipelines.

==> experiment.tex <==
\section{Preliminary Results}
\label{sec:results}

This section reports some preliminary results that estimates the error resilience characteristics of the MM with different \fp precision data types. 

\textbf{Fault Injection Methodology} We use the enhanced NVBitFI to conduct large-scale fault injection campaigns on four benchmarks from cutlass, namely volta-fp16-gemm, ampere-tf32-gemm and ampere-bf16-gemm and ampere-fp16-gemm. We run 1,000 fault injections for each configuration. For each fault injection trial, NVBitFI randomly chooses a kernel, a thread in that kernel, a \hmma instruction executed by the thread, a random destination register of that \hmma instruction, and a random term contributing to the result stored in that register. Note that for \tf the total number of the terms is eight while for \bft and \half it is 16. When a term is selected, NVBitFI conducts two sets of experiments: 1) to flip a random bit in its resulting \fp value as the baseline, and 2)  to flip a bit in a specific position of the \fp value, and estimate the priority of the bits in terms of their significance to the MM correctness. Once a bit is flipped, NVBitFI applies the ``write-back" approach to plant 
the erroneous value to the destination register of the \hmma instruction. 

\textbf{Fault Injection Results} Figure~\ref{fig:result} shows the fault injection results for GEMMs implemented with different \fp formats. The outcomes of the MM are categorized as SDC (i.e. the result fails the cutlass's default correctness check\footnote{cutlass calls \textit{TensorEquals}~\cite{tensorsqueal} utility functions to compare two tensors elementwise.}) or Benign (i.e. the result passes the check). The main take-aways are:
\begin{itemize}
\renewcommand{\labelitemi}{\scriptsize$\blacksquare$}
    \item \tf and \bft present similar trend of error resilience: (1) in both the formats the first exponent bits (MSB) are most vulnerable to faults; (2) the rest of bit positions behave similarly in terms of error resilience. 
    \item However, \bft in general shows much higher resilience to faults than \tf as the SDC rates are around 20\% while on \tf the SDC rates are around 60\%.
    \item For \half, faults in mantissa bits are more likely to lead to correct results than in exponent bits. This trend persists on both architectures for \half based GEMM. Based on the results, A100 seems to be more resilient to faults, but investigating the reasons for the difference between the architectures is part of our future work.
    % \siva{Interesting finding. I wonder why you are seeing this behavior. I assume the size of the GEMM and the input is the same on the two architectures?} 
\end{itemize}

\begin{figure*}[h]
    \vspace{-0.5cm}
     \centering
     \begin{subfigure}[t]{0.32\linewidth}
        \centering
         \includegraphics[width=\textwidth]{tf32_a100.pdf}
        %\caption{}
        %\label{fig:mpi_init}
     \end{subfigure}
     \hfill
     %\vspace{-0.2cm}
    \begin{subfigure}[t]{0.32\linewidth}
         \centering
         \includegraphics[width=\textwidth]{bf16_a100.pdf}
         %\caption{}
         %\label{fig:mpi_comm0}
     \end{subfigure}
          % \hfill
     %\vspace{-0.1cm}
     \begin{subfigure}[t]{0.32\linewidth}
         \centering
         \includegraphics[width=\textwidth]{fp16_a100.pdf}
         %\caption{}
        % \label{fig:mpi_comm1}
     \end{subfigure}
          \hfill
     \begin{subfigure}[t]{\linewidth}
       \centering
         \includegraphics[width=0.32\textwidth]{fp16_v100.pdf}
         %\label{fig:mpi_full}
     \end{subfigure}
     \vspace{-2em}
     %
     \caption{The fault injection results for the four benchmark GEMM with different \fp formats.}
      \vspace{-2em}
     \label{fig:result}
\end{figure*}



==> futurework.tex <==
\section{Future directions}
Our fault injection study demonstrates that different \fp formats exhibit distinct error resilience characteristics against hardware faults. This observation enables two future directions: 1). One needs to propose a format-specific approach to detect if an error occurred during the execution. The likelihood of a fault causing a failure during \bft based MM is the lowest among all the \fp formats, so that it is promising to relax the certain \fp checks for such format to trade for more efficient \fp computation; 2). It is interesting to understand how an incorrect MM impacts the correctness of an end-to-end application taking advantage of Tensor Cores, such as deep neural networks. Specifically, for a particular \fp format or the mixed-used \fp formats across different layers of a neural network, how do the different inherent masking abilities of these formats influence the accuracy of the DNN? We will investigate these directions in future work. 

==> hpca-template.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%% -- DO NOT MODIFY -- %%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\author{
  \ifdefined\hpcacameraready
    \IEEEauthorblockN{\hpcaauthors{}}
      \IEEEauthorblockA{
        \hpcaaffiliation{} \\
        \hpcaemail{}
      }
  \else
    \IEEEauthorblockN{\normalsize{HPCA \hpcayear{} Submission
      \textbf{\#\hpcasubmissionnumber{}}} \\
      \IEEEauthorblockA{
        Confidential Draft \\
        Do NOT Distribute!!
      }
    }
  \fi 
}

% Heading and footer for title page
\fancypagestyle{camerareadyfirstpage}{%
  \fancyhead{}
  \renewcommand{\headrulewidth}{0pt}
  \fancyhead[C]{
    \ifdefined\aeopen
    \parbox[][12mm][t]{13.5cm}{\hpcayear{} IEEE International Symposium on High-Performance Computer Architecture (HPCA)}    
    \else
      \ifdefined\aereviewed
      \parbox[][12mm][t]{13.5cm}{\hpcayear{} IEEE International Symposium on High-Performance Computer Architecture (HPCA)}
      \else
      \ifdefined\aereproduced
      \parbox[][12mm][t]{13.5cm}{\hpcayear{} IEEE International Symposium on High-Performance Computer Architecture (HPCA)}
      \else
      \parbox[][0mm][t]{13.5cm}{\hpcayear{} IEEE International Symposium on High-Performance Computer Architecture (HPCA)}
    \fi 
    \fi 
    \fi 
    \ifdefined\aeopen 
      \includegraphics[width=12mm,height=12mm]{ae-badges/open-research-objects.pdf}
    \fi 
    \ifdefined\aereviewed
      \includegraphics[width=12mm,height=12mm]{ae-badges/research-objects-reviewed.pdf}
    \fi 
    \ifdefined\aereproduced
      \includegraphics[width=12mm,height=12mm]{ae-badges/results-reproduced.pdf}
    \fi
  }
  %\fancyfoot[L]{\hpcapubid{} \copyright \hpcayear{} IEEE}
  \fancyfoot[C]{}
}
% Heading and footer for remaining pages
\fancyhead{}
\renewcommand{\headrulewidth}{0pt}
%\fancyhead[C]{\hpcayear{} IEEE International Symposium on
% High-Performance Computer Architecture (HPCA)}


\begin{document}
\maketitle

%Enables the camera ready header and footer
\ifdefined\hpcacameraready 
  \thispagestyle{camerareadyfirstpage}
  \pagestyle{empty}
\else
  \thispagestyle{plain}
  \pagestyle{plain}
\fi

\newcommand{\hpcaheight}{0mm}
\ifdefined\eaopen
\renewcommand{\hpcaheight}{12mm}
\fi
  

